Navigating Time's Possibilities: Plausible Counterfactual Explanations for Multivariate Time-Series Forecast through Genetic Algorithms

Counterfactual learning has become promising for understanding and modeling causality in complex and dynamic systems. This paper presents a novel method for counterfactual learning in the context of multivariate time series analysis and forecast. The primary objective is to uncover hidden causal relationships and identify potential interventions to achieve desired outcomes. The proposed methodology integrates genetic algorithms and rigorous causality tests to infer and validate counterfactual dependencies within temporal sequences. More specifically, we employ Granger causality to enhance the reliability of identified causal relationships, rigorously assessing their statistical significance. Then, genetic algorithms, in conjunction with quantile regression, are used to exploit these intricate causal relationships to project future scenarios. The synergy between genetic algorithms and causality tests ensures a thorough exploration of the temporal dynamics present in the data, revealing hidden dependencies and enabling the projection of outcomes under hypothetical interventions. We evaluate the performance of our algorithm on real-world data, showcasing its ability to handle complex causal relationships, revealing meaningful counterfactual insights, and allowing for the prediction of outcomes under hypothetical interventions.

==> Text/3method_old.tex <==

\section{Proposed Approach}
\emergencystretch 3em

Let $f$ be a model trained to solve a multi-variate time-series problem, in which the goal is to predict the value of a target variable based on a set of input features, where both the target variables and input features are time-dependent. To build $f$ we learn the mapping between the input features and the target variables based on historical data, which can be described as

\begin{equation}
{\hat{\mathcal{Y}}} = f({\mathcal{X}}; {\Theta})
\end{equation}


where $f(\cdot)$ represents the learned model, and ${\Theta}$ represents the parameters of the model. The model takes the input features ${\mathcal{X}}$ as input and produces predictions ${\hat{\mathcal{Y}}}$ for the target variable.

To predict future scenarios, we can further create an auto-regressive $f^{x}\cdot)$ model for each input variable $x \in {\mathcal{X}}$. By forecasting each variable $N-1$ steps into the future and using it as inputs to $f\cdot)$, we can obtain a forecast of ${\hat{\mathcal{Y}}}_N$ that describes the target variable $N$ steps into the future. 




However, if a specific ${y}_{goal}$ outcome is desired - such as the case in counterfactual explanations - we need to find a future scenario $\mathcal{X}'$ that leads to %{\hat{\mathcal{Y}}_N} \approx {\mathcal{Y}}_{goal}$. That is, 
$|{\hat{\mathcal{Y}}_N} - {\mathcal{Y}}_{goal}| \leq \epsilon$, $\epsilon$ being some low error tolerance margin.

Thus, the proposed approach consists of first creating individual models capable of generating synthetic time series. We propose training an independent model for each input variable, using past historical data and optimizing the pinball loss \citep{steinwart2011estimating}. The pinball loss, also known as quantile loss or quantile regression loss, is a loss function commonly used in quantile regression. It is specifically designed to measure the accuracy of quantile predictions, which estimate the conditional quantiles of a target variable given the input features.

In quantile regression, instead of predicting a single-point estimate, the goal is to estimate a range of quantiles. The pinball loss is used to evaluate how well the predicted quantiles match the actual quantiles of the target variable. The pinball loss is defined as follows for a given quantile level $\tau$ (ranging between 0 and 1) and a target variable $x$:

\begin{equation}
\mathcal{L}(\tau, x) = \max(\tau \cdot (x - x_{\text{pred}}), (\tau - 1) \cdot (x_{\text{pred}} - x))
\end{equation}


where $x_{\text{pred}}$ represents the predicted value for the target variable $x$. The pinball loss penalizes underestimations when $x$ is above $x_{\text{pred}}$ (positive error) and overestimations when $x$ is below $x_{\text{pred}}$ (negative error), with the magnitude of the penalty increasing as $\tau$ moves away from 0.5. By minimizing the pinball loss, quantile models can learn to provide accurate and reliable quantile estimates across different levels, capturing the full distributional information of the target variable. In the problem of building future scenarios, we can use these models to induce many plausible scenarios by using auto-regressive models with different quantiles. 

The proposed counterfactual algorithm aims to find, among the possible projections, the one that leads to the desired scenario. We can describe a future scenario as a $t$-shaped vector, where $t = |X|*N$. Each index corresponds to the probability (quantile) used to obtain the forecast of $x\in X$ for each time state $n \in N$. We can employ a genetic algorithm that searches for the probability sequence associated with the curve of each variable that approximates ${y}_{goal}$. Many fitness functions could be employed. A possibility might be the loss function proposed by \cite{back2020parallel}, a four-objective loss function for counterfactual explanations that established a multiobjective Pareto front:

\begin{equation}
\begin{split}
    \mathcal{L}(X, X', y_{goal}, X_{obs}) = \\
    (o_1(\hat{f}(X'), y_{goal}), o_2(X, X'), o_3(X, X'), o_4(X', X_{obs}))
\end{split}
\end{equation}

The first objective, $o_1$, aims to minimize the distance between the predicted counterfactual $\hat{f}(X')$ and the desired prediction $y_{goal}$. The second objective, $o_2$, measures the similarity between the counterfactual $X'$ and the original instance $X$, the present scenario. The third objective, $o_3$, counts the number of features that differ between $X$ and $X'$. By minimizing $o_3$, the goal is to achieve sparse feature changes. The fourth objective, $o_4$, evaluates the likelihood of the counterfactual $X'$. Each objective captures a specific criterion: proximity to the desired prediction, similarity to the original instance, sparsity of feature changes, and the likelihood of feature values/combinations \citep{molnar2020interpretable}.

Overall, we hypothesize that the counterfactual method described could allow for a better understanding of the projections of a time-series model and the variables that drive future scenarios. Furthermore, the use of synthetic time series anchored in historical data helps ensure that the created scenarios are realistic and plausible.


\subsection{Data}
